Property Checking Without Inductive Invariants

We introduce a procedure for proving safety properties. This procedure is based on a technique called Partial Quantifier Elimination (PQE). In contrast to complete quantifier elimination, in PQE, only a part of the formula is taken out of the scope of quantifiers. So, PQE can be dramatically more efficient than complete quantifier elimination. The appeal of our procedure is twofold. First, it can prove a property without generating an inductive invariant. Second, it employs depth-first search and so can be used to find deep bugs.

==> p3qe.tex <==
\section{Algorithm For Partial Quantifier Elimination}
\label{app:pqe}
In this section, we discuss Partial Quantifier Elimination (PQE) in
more detail. In Subsection~\ref{app_s:pqe_alg}, we give a high-level
description of a PQE-solver. This PQE-solver is based on the machinery
of Dependency sequents (D-sequents) that we recall in
Subsection~\ref{app_s:dep_seqs}.

%
% Subsection: PQE algorithm
%
\subsection{High-level description of a PQE solver}
\label{app_s:pqe_alg}

In this subsection, we describe an algorithm for PQE introduced
in~\cite{hvc-14} in 2014.  We will use the same name for this
algorithm as in Section~\ref{sec:experiments}, i.e. PQE-14.  Let
$A(V,W), B(V,W)$ be Boolean formulas where $V$,$W$ are non-overlapping
sets of variables. As we mentioned in Subsection~\ref{subsec:pqe_def},
the PQE problem is to find formula $A^*(V)$ such that
\pqe{W}{A}{A^*}{B}. We will refer to a clause containing a variable of
$W$ as a \pnt{W}\tb{-clause}. PQE-14 is based on the three ideas
below. 

\ti{First}, finding formula $A^*$ comes down to generation of clauses
depending only on variables of $V$ that make the $W$-clauses of $A$
redundant in $A^* \wedge \prob{W}{A \wedge B}$.  \ti{Second}, the
clauses of $A^*$ can be derived by resolving clauses of $A \wedge
B$. The intermediate resolvents that are $W$-clauses need to be proved
redundant along with the original $W$-clauses of $A$.  However, since
formula $B$ remains quantified, there is no need to prove redundancy
of $W$-clauses of $B$ or $W$-clauses obtained by resolving only
clauses of $B$.


\ti{Third}, since proving redundancy of a clause is a hard problem,
PQE-14 uses branching. After proving redundancy of required clauses in
subspaces, the results of branches are merged. The advantage of
branching is that for every $W$-clause $C$ one can always reach a
subspace where $C$ can be trivially proved redundant. Namely, $C$ is
trivially redundant in the current subspace if a) $C$ is satisfied in
the current branch; b) $C$ is implied by some other clause; c) there
is an unassigned variable $y$ of $C$ where $y \in W$, such that $C$
cannot be resolved on $y$ with other clauses that are not satisfied or
proved redundant yet.


%
% Subsection: Dependency sequents
%
\subsection{Dependency sequents}
\label{app_s:dep_seqs}
PQE-14 branches on variables of $V \cup W$ until the $W$-clauses that
are descendants of $W$-clauses of $A$ are proved redundant in the
current subspace. To keep track of conditions under which a $W$-clause
becomes redundant in a subspace, PQE-14 uses the machinery of
Dependency sequents (D-sequents) developed
in~\cite{fmcad12,fmcad13}. A \tb{D-sequent} is a record of the form
\Dss{W}{A \wedge B}{q}{\s{C}}. It states that clause $C$ is redundant
in formula \prob{W}{A \wedge B} in subspace \pnt{q}. Here \pnt{q} is
an assignment to variables of $V \wedge W$ and $A$ is the \ti{current}
formula that consists of the initial clauses of $A$ and the resolvent
clauses.  When a $W$-clause $C$ is proved redundant in a subspace,
this fact is recorded as a D-sequent. If $\pnt{q}=\emptyset$, the
D-sequent is called \ti{unconditional}. Derivation of such a D-sequent
means that clause $C$ is redundant in the current formula \prob{W}{A
  \wedge B} in the whole space.

The objective of PQE-14 is to derive unconditional D-sequents for all
$W$-clauses of $A$ and their descendants that are $W$-clauses.  A new
D-sequent can be obtained from two parent D-sequents by a
resolution-like operation on a variable $y$. This operation is called
\ti{join}. When PQE-14 merges the results of branching on variable $y$
it joins D-sequents obtained in branches $y=0$ and $y=1$ at variable
$y$.  So the resulting D-sequents do not depend on $y$.  If formula $A
\wedge B$ is unsatisfiable in both branches, a new clause $C$ is added
to formula $A$. Clause $C$ is obtained by resolving a clause falsified
in subspace $y=0$ with a clause falsified in subspace $y=1$ on
$y$. Adding $C$ makes all $W$-clauses redundant in the current
subspace.  By the time PQE-14 backtracks to the root of the search
tree, it has derived unconditional D-sequents for all $W$-clauses of
the current formula $A$.

PQE solving is work in progress and so is still lacking some important
techniques like D-sequent re-using.  In current algorithms, the parent
D-sequents are discarded as soon as they produce a new D-sequent by
the join operation. Although D-sequent re-using promises to be as
powerful as re-using learned clauses in SAT-solving, it requires more
sophisticated bookkeeping and so is not implemented yet~\cite{hvc-14}.


==> s0torage.tex <==
%
% Proposition: main LoRT
%
\begin{proposition}
\label{prop:main_lort}
Let \Et be a state transition system with stuttering specified by
transition relation $T$ and initial states $I$. Let $P$ be a property
to be verified.  Let the following conditions hold
\begin{itemize}
\item \impl{I_0 \wedge \Abs{T}{j-1}}{P} 
\item  $\prob{\Abs{S}{j}}{I_0 \wedge \Abs{T}{j}} \equiv \prob{\Abs{S}{j}}{I_1 \wedge \Abs{T}{j}}$ where $I_0 \ueqv I_1$.
\end{itemize}
Then property $P$ holds for  \et
\end{proposition}
%
%
\begin{proof}[\kern-10pt Proof] Let us prove by induction that 
$\prob{\Abs{S}{k}}{I_0 \wedge \Abs{T}{k}} \equiv \prob{\Abs{S}{k}}{I_{k+1-j} \wedge \Abs{T}{k}}$ where $I_0 \ueqv I_{k-j}$ for every $k > j$.

\vspace{5pt}
\noindent\ti{Base step}. 

\vspace{5pt}
\noindent\ti{Induction step}. The induction hypothesis is that
$\prob{\Abs{S}{k}}{I_0 \wedge \Abs{T}{k}} \equiv \prob{\Abs{S}{k}}{I_{k+1-j} \wedge \Abs{T}{k}}$
where $I_0 \ueqv I_{k-j}$ implies that
$\prob{\Abs{S}{k+1}}{I_0 \wedge \Abs{T}{k+1}} \equiv \prob{\Abs{S}{k+1}}{I_{k+2-j} \wedge \Abs{T}{k+1}}$
where $I_0 \ueqv
I_{k+1-j}$. Denote \prob{\Abs{S}{k+1}}{I_0 \wedge \Abs{T}{k+1}}
as \Fi. Formula \Fii can be represented
as \Prob{S_{k+1}}{\Abs{S}{k}}{I_0 \wedge \Abs{T}{k} \wedge
T_{k+1,k+2}}. Since $T_{k+1,k+2}$ does not depend on variables
of \Abs{S}{k} formula \Fii can be rewritten as
$\exists{S_{k+1}}[T_{k+1,k+2} \wedge \prob{\Abs{S}{k}}{I_0 \wedge \Abs{T}{k}}]$.
Using the induction hypothesis \Fii can be transformed into
$\exists{S_{k+1}}[T_{k+1,k+2} \wedge \prob{\Abs{S}{k}}{I_{k+1-j} \wedge \Abs{T}{k}}]$.
After moving $T_{k+1,k+2}$ under the scope of quantifiers we obtain
$\exists{S_{k+1}}[\prob{\Abs{S}{k}}{I_{k+1-j} \wedge \Abs{T}{k+1}}]$. By
changing the order of quantifiers we get
$\exists{\Abs{S}{k-j}}[\prob{\Abs{S}{k+1-j,k+1}}{I_{k+1-j} \wedge \Abs{T}{k+1}}]$.
Taking into account the stuttering feature of \Et, this formula can be
represented as $\exists{\Abs{S}{k-j}}[\Abs{T}{k-j} \wedge
\prob{\Abs{S}{k+1-j,k+1}}{I_{k+1-j} \wedge \Abs{T}{k+1-j,k+1}}]$.

Using variable renaming and the fact that  
$\prob{\Abs{S}{j}}{I_0 \wedge \Abs{T}{j}} \equiv \prob{\Abs{S}{j}}{I_1 \wedge \Abs{T}{j}}$
formula $\prob{\Abs{S}{k+1-j,k+1}}{I_{k+1-j} \wedge \Abs{T}{k+1-j,k+1}}]$
can be represented as $\prob{\Abs{S}{k+1-j,k+1}}{I_{k+2-j} \wedge \Abs{T}{k+1-j,k+1}}]$.
So formula \Fii can be rewritten as $\exists{\Abs{S}{k-j}}[\Abs{T}{k-j} \wedge
\prob{\Abs{S}{k+1-j,k+1}}{I_{k+2-j} \wedge \Abs{T}{k+1-j,k+1}}]$. Putting
\Abs{T}{k-j} back under the scope of quantifiers we get formula
\prob{\Abs{S}{k+1}}{I_{k+2-j} \wedge \Abs{T}{k+1}} that is equivalent
to the original formula \Fi.
\end{proof}
------
\begin{proposition}
\label{prop:bad_state}
Let $H(S_{j+1})$ be a formula such that $\prob{\Abs{S}{j}}{I_0 \wedge
  I_1 \wedge \Abs{T}{j+1} \wedge \overline{P}} \equiv H \wedge
\prob{\Abs{S}{j}}{I_0 \wedge \Abs{T}{j+1} \wedge \overline{P}}$.
Then a bad state \pnt{s_{j+1}} is reachable for the first time in $(j+1)$-th
time iff 
\begin{itemize}
\item $H(\pnt{s_{j+1}})=0$ and 
\item \nimpl{I_0 \wedge \Abs{T}{k+1}}{H} 
\end{itemize}
\end{proposition}
-----
 Note that
a tradictional approach to finding the diameter of \Ks requires
\ti{complete} QE of \prob{\Abs{S}{n}} {I_0 \wedge \Abs{T}{n}}. This
can be drastically more complex than PQE because one needs to take
\ti{the entire formula} out of the scope of quantifiers.
--------
One of the most popular approaches of checking if a new bad state is
reachable in $n$-th time frame is Bounded Model Checking (BMC). In
BMC, one checks for satisfiability formula $I_0 \wedge \Abs{T}{n}
\wedge \overline{P_n}$. Informally, one can view SAT as a special case
of complete QE where all variables are quantified. So in BMC the
entire formula formula has to be taken out of the scope of
quantifiers.  In particular, if $I_0 \wedge \Abs{T}{n} \wedge
\overline{P_n}$ is unsatisfiable, one has to derive an empty clause
that makes \ti{all clauses} of this formula redundant. By contrast,
\NBS needs to prove \ti{only} the redundancy of formula $I_1$. A
trivial way to do this is to follow the BMC guidlines i.e. to show
that $I_0 \wedge \Abs{T}{n} \wedge \overline{P_n}$ implies an empty
clause that subsumes $I_1$.  \NBS has the potential of proving
redundancy of $I_1$ in a much more efficient way by using the
machinery of Dependency sequents (D-sequents) we developed
in~\cite{fmcad12,fmcad13}.  In particular, this machinery allows one
to prove redundancy of $I_1$ without generation of an empty clause. 
------------
 When processing $i$-th time, \ST first calls \NBS to find a
bad state reachable only in at least $i$ transitions.  If \NBS
succeeds, \ST reports that property $P$ fails. Otherwise, \ST calls
\NS to find a new good state.  If \NS fails, \ST reports that property
$P$ holds. Otherwise it increments the value of $i$ by 1 and starts a
new iteration.
-------------
 A
traditional way to check if a new state is reached in $n$-th time
frame is based on breadth-first search. That is one has to
consecutively compute the set of states of reachable in
$1,2,\dots,n-1$ transitions before deciding if a new state is
reachable in $n$-th time frame. Needless to say that such an approach
can be extremely expensive. By contrast, as we show in
Section~\ref{sec:dfs}, the fact that \NS is based on PQE makes it
possible to look for a state that is reachable only in $n$ transitions
in a depth-first manner.
----------
Note that the situation is aggrevated by the fact that BMC
solves a harder problem than \NBS because it cannot ignore states
reachable in earlier time frames. In other words, BMC tries to find a
bad state no matter whether it is new or is reachable in an earlier
time frame.  So a SAT-solver cannot backtrack from the subspace that
contains only states reachable in before $n$-th time frame. 
-------
 Another way to contrast complete
quantifier elimination with PQE is as follows.  The former deals with
a single formula and so, in a sense, has to cope with its
\ti{absolute} complexity. By contrast, PQE operates on two formulas
($A$ and $A \wedge B$) and its efficiency depends on their
\ti{relative} complexity.  This is important because no matter how
high the individual complexity of these formulas is, their relative
complexity can be quite manageable.
---------
We introduce a new method for checking safety properties that does not
require generation of inductive invariants.  This method is based on a
new procedure called \cd. It checks if the diameter is reached i.e. if
a state not seen before is reachable in $n$-th time frame.  This check
is performed by a technique called partial quantifier elimination. We
also describe a modification of \CD called \BS that checks if a bad
state not seen so far is reachable in $n$-th time frame.  One can
prove that a property holds without generating an inductive invariant
by unrolling the transition relation and applying \BS and \cd. First,
\BS is called to find a bad state reached in $n$-th time frame. If it
fails, \CD is invoked to check if a new good state is reached in
$n$-th time frame. The convergence of this method can be drastically
sped up by combining the procedure above with expansion of the set of
initial states.  The expanded set is gradually tightened up until a
counterexample is generated by \BS or the property at hand is proved
by \cd.
--------
%
% Subsection: Finding diameter PQE
%
\subsection{Finding diameter by PQE}
Let $S_i$ denote the set of state variables of $i$-th time frame.  Let
\Abs{S}{j} denote $S_0 \cup \dots \cup S_j$. Let \Abs{T}{j} denote
$T(S_0,S_1) \wedge \dots \wedge T(S_{j-1},S_j)$. Checking if $n \geq
\di{\ks}$ comes down to finding out if \KS reaches a new state in
$n$-th iteration (i.e. a state that cannot be reached in a fewer
number of transitions).  In this paper we introduce a procedure called
\CD that performs this check.  \CD operates by checking redundancy of
formula $I_1$ in \prob{\Abs{S}{n-1}}{I_0 \wedge I_1 \wedge \Abs{T}{n}}
where $I_0=I(S_0)$ and $I_1 = I(S_1)$. That is it verifies if
$\prob{\Abs{S}{n-1}}{I_0 \wedge I_1 \wedge \Abs{T}{n}} \equiv
\prob{\Abs{S}{n-1}}{I_0 \wedge \Abs{T}{n}}$. If so, no new state can
be reached in $n$-th iteration and $n$ exceeds \di{\ks}.  Checking
redundancy of $I_1$ is an instance of the PQE problem because only
formula $I_1$ needs to be taken out of the scope of quantifiers.

Here is an informal explanation of why \CD is correct.  The set of
states reachable in $n$ transitions is specified by
\prob{\Abs{S}{n-1}}{I_0 \wedge \Abs{T}{n}}. Adding $I_1$ to this
formula shortcuts the initial time frame and so
\prob{\Abs{S}{n-1}}{I_0 \wedge I_1 \wedge \Abs{T}{n}} specifies the
set of states reachable in $n-1$ transitions. The fact that $I_1$ is
redundant means that the sets of states reachable in $n$ and $n-1$
transitions are the same.

%
% Subsection: finding a bad state by PQE
%
\subsection{Finding a bad state by PQE}
Let $P$ be a formula specifying the property of \KS to be proved.
Suppose that one needs to check if a bad state is reached in $n$-th
time frame for the first time. (That is this state cannot be reached
in an earlier time frame.) Using the reasoning above one can show that
this problem comes down to checking if formula $I_1$ is redundant in
\prob{\Abs{S}{n-1}}{I_0 \wedge I_1 \wedge \Abs{T}{n} \wedge
  \overline{P_n}} where $P_n = P(S_n)$. If $I_1$ is redundant, then no
new bad state is reached in $n$-th time frame. We will refer to the
procedure for solving the PQE problem above as \bs. Note that \BS is
just a variation of \CD that looks only for a new \ti{bad} state.
--------
Suppose that one needs to check that a property $P$ of a sequential
circuit $M$ holds. Let $T$ be the transition relation specified by $M$
and \KS be the transition system defined by $T$ and a formula $I$
specifying the initial states (see Subsection~\ref{subsec:problem}).
---------
If \KS does not have this feature, one can
introduce stuttering by adding to circuit $M$ a combinational input
variable $v$.  The modified circuit $M$ works as before if $v=1$ and
copies its current state to the output state variables if $v=0$
-----------
%
% Subsection: two ways to solve the RD problem
%
\subsection{Two methods for finding the reachability diameter}
\label{ssec:two_impl}
In this paper, we consider two methods of solving the RD problem using
the idea of Subsection~\ref{ssec:main_idea}.  One method is to check
if $I_1$ is redundant in \prob{\Abs{S}{n}}{I_0 \wedge I_1 \wedge
  \Abs{T}{n+1}} for consecutive values of $n$ starting with $n=2$. If
making $I_1$ redundant requires adding at least one clause
$C(S_{n+1})$ that is implied by $I_0 \wedge I_1 \wedge \Abs{T}{n+1}$
but not $I_0 \wedge \Abs{T}{n+1}$, then $\di{I,T} > n$. That is
proving $\di{I,T} > n$, does not require generation of all states
reachable in $n$ transitions. In other words, PQE facilitates
\ti{depth-first search}.  In more detail this topic is discussed in
Section~\ref{sec:dfs}.

The second method of solving the RD problem is as follows. Let
$H_i(S_i)$, $i=1,\dots,n$ be a set of formulas such that $H_1$ is a
subset of clauses of $I_1$ and formula $H_i$, $i=2,\dots,n$ is
obtained by resolving clauses of $I_0 \wedge I_1 \wedge \Abs{T}{i}$.
One can view formulas $H_1,\dots,H_n$ as a result of ``pushing''
clauses of $I_1$ to later time frames.  The main property satisfied by
these formulas is that $\prob{\Abs{S}{n-1}}{I_0 \wedge I_1 \wedge
  \Abs{T}{n}} \equiv H_n \wedge \prob{\Abs{S}{n-1}}{I_0 \wedge
  \Abs{H}{n-1} \wedge \Abs{T}{n}}$ where $\Abs{H}{n-1} = H_1 \wedge
\dots \wedge H_{n-1}$.

The second method starts with $n=1$ and $H_1 = I_1$.  At every step it
picks a clause of $H_n$ and replaces it with a set of clauses
$H_{n+1}(S_{n+1})$. This method is based on the observation that if $n
= \di{I,T}$, any clause $C(S_{n+1})$ that is a descendent of $I_1$ is
implied by $I_0 \wedge \Abs{T}{n+1}$. So one does not need to add
clauses depending on $S_{n+1}$ to make formula $H_n$ redundant. In
other words, pushing the descendents of $I_1$ to later time frames
inevitably results in making them redundant. The value of \di{I,T} is
given by the largest index $n$ of a time frame where a descendent of
$I_1$ was not redundant yet.
-------
\FB solves these problems \ti{together}. (For the sake of simplicity,
when introducing \FB in Subsection~\ref{ssec:pc_no_inv}, we said that
it \ti{partitions} the safety problem into these two problems.)
----------
We introduce two new procedures for checking safety properties called
\FB and \pp. The appeal of these procedures is that they do not
require generation of inductive invariants. \FB and \PP are based on a
technique call Partial Quantifier Elimination (PQE). Namely, we show
that computing the reachability diameter reduces to PQE. In contrast
to complete quantifier elimination, in PQE, only a part of the formula
is taken out of the scope of quantifiers. So PQE can be dramatically
more efficient than complete quantifier elimination. One more
attraction of PQE is that it facilitates depth-first search.  Both \FB
and \PP are complete procedures. \FB is meant for finding deep bugs
whereas \PP is aimed at faster convergence when proving that a
property holds.
----------
\FB is a complete procedure, it is either proves that $P$
holds or finds a counterexample. \FB is tailored to finding deep bugs
by employing depth-first search.

If property $P$ holds and \di{I,T} is large, the \FB procedure may
converge too slowly.  We describe procedure \PP that addresses this
problem by using an expanded set of initial states \Sup{I}{exp}. The
\PP procedure partitions the safety problem into the following two
subproblems.
\begin{enumerate}
\item Find value $n$ and formula \Sup{I}{exp} such that 
\begin{enumerate}[a)]
\item \impl{I}{\Sup{I}{exp}} and \impl{\Sup{I}{exp}}{P}
\item  $n \geq \di{\Sup{I}{exp},T}$
\end{enumerate}
\item Check that \impl{\rch{\Sup{I}{exp},T,n}}{P}.
\end{enumerate}
Note that the value of $n$ can be much smaller than \di{I,T}. In
particular, if $n=1$, then \Sup{I}{exp} is an inductive invariant.
----------
Usually the RD problem is solved by
eliminating quantifiers either explicitely (by applying a QE
algorithm) or implicitely (by solving the RD problem in terms of
quantifer-free formulas). 
----------
 Given a formula $B(S)$, we will call \pnt{s} a $B$-state if
$B(\pnt{s})=1$.
-------
As we showed in Subsection~\ref{ssec:main_idea}, to prove
$\mi{Diam}(I,T) \leq n$ one needs to show that formula $I_1$ redundant
is in \prob{\Abs{S}{n}}{I_0 \wedge I_1 \wedge \Abs{T}{n+1}}. So to
prove the opposite i.e.  $\mi{Diam}(I,T) > n$, it suffices to show the
existence of a state \pnt{s_{n+1}} that
\begin{enumerate}
\item is reachable in $(n+1)$-th time frame and 
\item is not reachable in $n$-th time frame
\end{enumerate}
%
(Since we consider systems with stuttering, the second condition
guarantees that \pnt{s} is not reachable in any time frame $m$ where
$m < n$.)

Given formula $I_0 \wedge I_1 \wedge \Abs{T}{n+1}$ one can satisfy
the two conditions above by 
\begin{enumerate}[a)]
\item finding a trace \tr{s}{0}{n+1} that satisfies $I_0 \wedge
  \Abs{T}{n+1}$
\item generating a clause $C$ implied by $I_1 \wedge T_{1,2} \wedge
  \dots \wedge T_{n,n+1}$ that is falsified by \pnt{s_{n+1}}.
\end{enumerate}
Condition a) proves \pnt{s_{n+1}} reachable in $(n+1)$-transitions.
Condition b) guarantees that \pnt{s_{n+1}} is not reachable in
$n$ transitions. 

Note that satisfying conditions a) and b) above \ti{does not require
  breadth-first search} i.e. computing the set of all states reachable
in $n$ transitions. In particular, clause $C$ of condition b) can be
found by taking $I_1$ out of the scope of quantifiers in
\prob{\Abs{S}{n}}{I_0 \wedge I_1 \wedge \Abs{T}{n+1}} (i.e. by solving
the PQE problem). Note that, in general, a solution to the PQE problem
above is implied by the entire formula $I_0 \wedge I_1 \wedge
\Abs{T}{n+1}$. On the other hand, condition b) requires clause $C$ be
implied by formula $I_1 \wedge T_{1,2} \wedge \dots
T_{n,n+1}$. However, the proposition below shows that this difference
does not matter.
%
\begin{proposition}
\label{prop:dfs}
Let \KS be an $(I,T)$-system and $H(S_{n+1})$ be a formula. Then $I_0
\wedge I_1 \wedge \Abs{T}{n+1} \rightarrow H$ entails $I_1 \wedge
T_{1,2} \wedge \dots T_{n,n+1} \rightarrow H$.
\end{proposition}


In the context of PQE-solving, condition a) requires $C$ not be
``noise'' i.e. not be implied by the part of the formula that remains
quantified (see Section~\ref{sec:pqe_def}). In this paper, we assume
that one employs PQE algorithms that may generate noise
clauses. (Note, however, that building a PQE-solver that does not
generate noise is quite possible~\cite{clean_pqe}.)  So, to make sure
that condition a) holds, one must prove $I_0 \wedge \Abs{T}{n+1}
\wedge \overline{C}$ satisfiable.
--------
(For the sake of simplicity, in the
introduction, we said that \PP \ti{partitions} the safety problem into
these two problems.)  


==> s1torage.tex <==
Importantly, there is a
strong relation between PQE and the notion of \ti{redundancy} of a
clause in a quantified formula. (A \tb{clause} is a disjunction of
literals.) In particular, solving the PQE problem above comes down to
finding a formula $A^*(V)$ implied by $A \wedge B$ that makes the
clauses of $A$ redundant in $A^* \wedge \prob{W}{A \wedge B}$. Then
$\prob{W}{A \wedge B} \equiv A^* \wedge \prob{W}{A \wedge B} \equiv
A^* \wedge \prob{W}{B}$.
---------
\begin{lemma}
\label{lemma:diam}
Let \KS be an $(I,T)$-system. Then $\di{I,T} \leq n$ iff
$\prob{\Abs{S}{n}}{I_0 \wedge \Abs{T}{n+1}} \equiv
\prob{\Abs{S}{n}}{I_1 \wedge \Abs{T}{n+1}}$ where $I_0 \ueqv I_1 \ueqv
I$ and $n \geq 0$.
\end{lemma}
------
\begin{proposition}
\label{prop:diam_pqe}
Let \KS be an $(I,T)$-system. Then $\di{I,T} \leq n$ iff formula $I_1$
is redundant in \prob{\Abs{S}{n}}{I_0 \wedge I_1 \wedge \Abs{T}{n+1}}
where $I_0 \ueqv I_1 \ueqv I$ (i.e.  iff $\prob{\Abs{S}{n}}{I_0 \wedge
  \Abs{T}{n+1}} \equiv \prob{\Abs{S}{n}}{I_0 \wedge I_1 \wedge
  \Abs{T}{n+1}}$).
\end{proposition}
------
\item Let $A(X')$ and $B(X'')$ be formulas where $X',X''$ are sets of
  variables such that $|X'| = |X''|$.  Then $A(X') \ueqv B(X'')$ means
  that $A$ and $B$ are equal modulo renaming variables. For instance,
  $I \ueqv I_0 \ueqv I_1$ holds.
---------  
Given number $n$, the RD problem is to find the value of predicate
$\di{I,T} \leq n$. It reduces to checking if the sets of states
reachable in $n$ and $(n+1)$ transitions are identical. The latter, as
Proposition~\ref{prop:diam_pqe} below shows, comes down to checking if
formula $I_1$ is redundant in \prob{\Abs{S}{n}}{I_0 \wedge I_1 \wedge
  \Abs{T}{n+1}} i.e. whether $\prob{\Abs{S}{n}}{I_0 \wedge I_1 \wedge
  \Abs{T}{n+1}} \equiv \prob{\Abs{S}{n}}{I_0 \wedge \Abs{T}{n+1}}$. If
$I_1$ is redundant, then $\di{I,T} \leq n$.  This is a special case of
the PQE problem. Instead, of finding a formula $H(S_{n+1})$ such that
$\prob{\Abs{S}{n}}{I_0 \wedge I_1 \wedge \Abs{T}{n+1}} \equiv H \wedge
\prob{\Abs{S}{n}}{I_0 \wedge \Abs{T}{n+1}}$ one just needs to decide
if $H \equiv 1$.
---
These
procedures give one more evidence that development of efficient
PQE-algorithms is of great importance.
-------
The contribution of the paper is twofold. First, we introduce a new
method of property checking that does not require generation of an
inductive invariant. Second, we give one more evidence that
development of efficient PQE-algorithms is of great importance.
--------
Besides, in case property
$P$ holds, convergence of \PP depends on proximity of $P$ to an
inductive invariant even less than that of algorithm of
~\cite{tech_rep_pc_lor}. This is because \PP does not build an
explicit inductive invariant.
---------
In~\cite{tech_rep_pc_lor}, we showed how one can combine
transition relation relaxation and PQE to build inductive invariants
that may be far away from the property at hand.
----------
In spite of great progress in property checking, the existing methods
have at least two flaws. The first flaw is that they cannot find
``deep'' bugs. In case of complete algorithms of property checking,
this flaw is a consequence of breadth-first search employed by these
algorithms.  For instance, IC3 builds a sequence of formulas
$F_1,\dots,F_n$ where $F_i$ specifies a super-set of the set of states
reachable in $i$ transitions. Formula $F_i$ is built \ti{after}
formulas $F_1,\dots,F_{i-1}$ have been constructed i.e. in a
breadth-first manner. In case of BMC, the problem is as follows. To
build a counterexample of $n$ transitions, one needs to find an
assignment satisfying a formula whose size grows linearly with $n$.
So finding a counterexample for large values of $n$ is infeasible.

The second flaw is that the ability of existing methods to build an
inductive invariant is based on assumptions that do not always hold.
For instance, IC3 builds an inductive invariant by tightening up the
property $P$ to be proved. So an implicit assumption of IC3 is that
there is an inductive invariant that is close to $P$.  Interpolation
based methods extract an interpolant from a proof that a property
holds for a specified number of transitions. The quality of an
interpolant strongly depends on that of the proof it is extracted
from. So these methods work under the assumption that a SAT-solver can
generate a high-quality and structure-aware proof. In many cases, the
assumptions above do not hold. For instance, neither assumption above
holds for an instance of property checking specifying sequential
equivalence checking.  An inductive invariant may be very far away
from the property describing sequential equivalence and a conflict
driven SAT-solver builds proofs of poor quality for equivalence
checking formulas.
-------
\begin{tabbing}
// $\Abs{R}{n} = R_1 \wedge \dots \wedge R_n$ \\
// \\
aaa\=bb\=cc\= dd\= \kill
$\pp(I,T,P)$\{\\
\tb{\scriptsize{1}}\> $T := \mi{MakeStutter}(T)$; \\
\tb{\scriptsize{2}}\> $\mi{Cex} := \mi{Unsat}(I_0 \wedge T_{0,1} \wedge \overline{P})$; \\
\tb{\scriptsize{3}}\> if ($\mi{Cex} \neq \mi{nil}$) return($\mi{Cex}$); \\
\tb{\scriptsize{4}}\> $H_1 := I_1$; \\
\tb{\scriptsize{5}}\> $n := 1$; \\
$~~~~~~ ---------$ \\
\tb{\scriptsize{6}}\> while ($H_1 \not\equiv 1$) \{ \\
\tb{\scriptsize{7}}\Tt  if ($H_n \equiv 1$) \{ \\
\tb{\scriptsize{8}}\ttt    $n := n-1$; \\
\tb{\scriptsize{9}}\ttt     continue; \}\\
\tb{\scriptsize{10}}\Tt   if $(\mi{FirstVisit}(n+1))$ $R_{n+1} := 1$; \\[4pt]
%
\tb{\scriptsize{11}}\Tt   $C:= \mi{PickClause}(H_n)$; \\
\tb{\scriptsize{12}}\Tt   $H_n := H_n \setminus \s{C}$; \\
\tb{\scriptsize{13}}\Tt  $H_{n+1}:= \mi{PQE}(\prob{\Abs{S}{n}}{I_0 \wedge C \wedge \Abs{H}{n} \wedge \Abs{T}{n+1}})$; \\[4pt] 
%%
\tb{\scriptsize{14}}\Tt  $\mi{RemNoise}(H_{n+1},\Abs{R}{n+1},I,T)$;\\
\tb{\scriptsize{15}}\Tt  if ($H_{n+1} \equiv 1$) continue; \\
\tb{\scriptsize{16}}\Tt  $\mi{Cex} := \mi{ChkBadSt}(H_{n+1},\Abs{R}{n+1},I,T,P)$;\\
\tb{\scriptsize{17}}\Tt  if ($\mi{Cex} \neq \mi{nil}$) return($\mi{Cex}$); \\
\tb{\scriptsize{18}}\Tt  $n := n+1$; \} \\
$~~~~~~ ---------$ \\
\tb{\scriptsize{19}}\>  return($\mi{nil}$); \}\\
\end{tabbing}
-----------
+) mention that prove_prop implies that
      the diameter is not known. Otherwise,
      one can use BMC
--------      
\begin{enumerate}
\item Show that $\di{I,T} \leq n$ for some value of $n$ (i.e. solve
  the RD problem).
\vspace{3pt}
\item Check that \impl{\rch{I,T,n}}{P}.
\end{enumerate}
-----
%
\begin{enumerate}
\item Find value $n$ such that $n \geq \di{I,T}$.
\vspace{3pt}
\item Check that \impl{\rch{I,T,n}}{P}.
\end{enumerate}
--------
*) modify the subsection "finding the diameter"

*) mark the lines of the prove_prop procedure that needs
to be removed if one just needs to compute the diameter
---------
+) mention that the code of prove_prop minus marked
 lines finds the dimeter
---------- 
The RD problem can be easily formulated in
terms of quantified formulas.  Usually the RD problem is solved by
performing quantifier elimination.  In this paper, we show that the RD
problem can be cast as an instance of the PQE problem. So, to solve
the RD problem one actually needs to take only a small part of the
formula out of the scope of the quantifiers.
---------
(Such methods are developed under the assumption that an efficient PQE
algorithm will be finally built.)  ----
\begin{abstract}
We introduce \pp, a procedure for proving safety properties.  \PP is
based on a technique called Partial Quantifier Elimination (PQE).  In
contrast to complete quantifier elimination, in PQE, only a part of
the formula is taken out of the scope of quantifiers. So PQE can be
dramatically more efficient than complete quantifier elimination.  The
appeal of \PP is twofold. First, it can prove a property without
generating an inductive invariant. This is an implication of the fact
that computing the reachability diameter of a system reduces to
PQE. Second, PQE enables depth-first search, so \PP can be used to
find very deep bugs. To prove property true, \PP has to consider
traces of length up to the reachability diameter. This may slow down
property checking for systems with a large diameter. We describe a
variation of \PP that can prove a property without generation of long
traces.
\end{abstract}
--------
%
% Subsection: the merits of our approach
%
\subsection{The merits of \pp}
The merits of \PP are as follows.  \PP is based on PQE and as we
mentioned above, the latter can be dramatically \ti{more efficient
  than QE}. Importantly, employing PQE facilitates depth-first
search. This feature enables \PP to search for \ti{deep
  bugs}. Besides, due to depth-first search, \PP does not need to
compute the set of all states reachable in $n$ transitions to decide
if the diameter is reached. Probably, the most important advantage of
\PP is that is solves the RD problem in terms of quantified
formulas. So \PP and/or its variation \FC can potentially prove a
property when an inductive invariant is prohibitively large or too
difficult to find.
----------
+) remove mentioning that IC cannot find deep bugs
   +) add reference to IC3 with finding deep bugs
--------   
+) drop mentioning prove_prop*
---------------
*) mention that stuttering is not
   critical for the approach

*) define notion of rechability

*) write background 
   
    +) recurrence diameter

    +) my paper on range computation
----------    
*) mention that everything we say about
   performance of our procedures is predicated on
   the assumption that there is an efficient PQE algorithm.
--------
*) modify the section introducing PQE
  +) add reference to PQE by certificate clauses
  +) mention that we rely on existence of an efficient
     PQE solver
----------     
A summary
of our results on this topic published in
~\cite{fmcad12,fmcad13,hvc-14} can be found in~\cite{tech_rep_ec_lor}
-------------
(Note, however, that
building a noise-free PQE-solver is possible~\cite{clean_pqe}.)
--------
In~\cite{clean_pqe}, we describe a ``noise-free'' PQE algorithm.
-----------
A straightforward method of property checking is to use Quantifier
Elimination (QE) for computing reachable states.  Current QE
algorithms still have problems ranging from memory explosion (QE by
BDDs~\cite{bryant_bdds1}) to poor performance (QE by
SAT)~\cite{blocking_clause,andy,fmcad12,fmcad13,cmu}). So, the main
focus of research has shifted towards methods that avoid
QE~\cite{ken03,ic3}.

Nevertheless, we have at least two reasons to be optimistic about
developing efficient procedures for quantified formulas.  The first
reason is that in many cases QE can be replaced with Partial QE (PQE)
introduced in~\cite{hvc-14}. In contrast to QE, in PQE, only a (small)
part of the formula is taken out of the scope of quantifiers. So, PQE
can be dramatically more efficient than QE.  The list of problems
where one can effectively employ PQE includes combinational
equivalence checking~\cite{tech_rep_ec_lor},
simulation~\cite{tech_rep_ec_sim}, inductive invariant generation in
property checking~\cite{tech_rep_pc_lor}, computing states reachable
\ti{only} from a particular set of states~\cite{tech_rep_crr}. In this
paper, we expand this list with a procedure for property checking
without generation of an inductive invariant.  The second reason for
our optimism is the introduction of the machinery of
D-sequents~\cite{fmcad12,fmcad13,fmsd14}. This machinery has shown a
great promise for boosting algorithms on quantified formulas. In
particular, it allows one to exploit the power of transformations that
preserve equisatisfiability rather than equivalence with the original
formula.


==> s2torage.tex <==
%
%  Structure
%
\subsection{Structure of the paper}
This paper is structured as follows.  We recall PQE in
Section~\ref{sec:pqe_def}. Basic definitions and notation conventions
are given in Section~\ref{sec:defs}.  Section~\ref{sec:gist} describes
how one can look for a counterexample and solve the RD problem by PQE.
In Section~\ref{sec:dfs}, we show that PQE enables depth-first search
in property checking.  The \PP and \FC procedures are presented in
Sections~\ref{sec:prove_prop} and~\ref{sec:prove_prop*} respectively.
Section~\ref{sec:background} provides some background. We make
conclusions in Section~\ref{sec:conclusions}.
---------
Now, let us show that if \prob{\Abs{S}{n}}{I_1 \wedge \Abs{T}{n+1}}=1
under assignment \pnt{s_{n+1}}, then \prob{\Abs{S}{n}}{I_0 \wedge
  \Abs{T}{n+1}}=1 under assignment \pnt{s_{n+1}}.
---------  
First, let us show that if \prob{\Abs{S}{n}}{I_0 \wedge
  \Abs{T}{n+1}}=1 under assignment \pnt{s_{n+1}} to $S_{n+1}$, then
\prob{\Abs{S}{n}}{I_1 \wedge \Abs{T}{n+1}}=1 under assignment
\pnt{s_{n+1}}.
-------
In this paper, we present a new procedure for checking safety
properties called \pp.  It is based on a technique called Partial
Quantifier Elimination (PQE) and so the efficiency of \PP is
predicated on that of PQE.  This assumption is not far from the truth
due to two facts.  First, intuitively, PQE should be much more
efficient than regular quantifier elimination because only a small
part of the formula is taken out of the scope of quantifiers. Second,
in~\cite{fmcad12,fmcad13,cert_tech_rep}, we developed the machinery of
redundancy based reasoning meant for efficiently handling quantified
formulas (in particular PQE). The advantage of \PP is twofold. First,
due to using PQE, it enjoys depth-first search and so can be used for
finding very deep bugs.  Second, \PP can prove that a property holds
without generation of an inductive invariant. This may turn out to be
extremely useful when inductive invariants are prohibitively large or
are hard to find.
---
Second, the introduction of
the machinery of D-sequents has a promise of boosting the performance
of PQE even further.
-------
In the worst case, \FC will reduce \Sup{I}{exp} to
$I$.
-------
Let \rch{I,T,n} denote a formula specifying the set of states
reachable in an $(I,T)$-system in $n$ transitions.
-------
\begin{enumerate}
\item Find the value of \di{I,T}.
\vspace{3pt}
\item Check that \impl{\rch{I,T,n}}{P} where $n = \di{I,T}$.
\end{enumerate}

